Autonomous Navigation for Robot-assisted Intraluminal and Endovascular Procedures: A Systematic Review

Increased demand for less invasive procedures has accelerated the adoption of Intraluminal Procedures (IP) and Endovascular Interventions (EI) performed through body lumens and vessels. As navigation through lumens and vessels is quite complex, interest grows to establish autonomous navigation techniques for IP and EI for reaching the target area. Current research efforts are directed toward increasing the Level of Autonomy (LoA) during the navigation phase. One key ingredient for autonomous navigation is Motion Planning (MP) techniques. This paper provides an overview of MP techniques categorizing them based on LoA. Our analysis investigates advances for the different clinical scenarios. Through a systematic literature analysis using the PRISMA method, the study summarizes relevant works and investigates the clinical aim, LoA, adopted MP techniques, and validation types. We identify the limitations of the corresponding MP methods and provide directions to improve the robustness of the algorithms in dynamic intraluminal environments. MP for IP and EI can be classified into four subgroups: node, sampling, optimization, and learning-based techniques, with a notable rise in learning-based approaches in recent years. One of the review's contributions is the identification of the limiting factors in IP and EI robotic systems hindering higher levels of autonomous navigation. In the future, navigation is bound to become more autonomous, placing the clinician in a supervisory position to improve control precision and reduce workload.

==> table4.tex <==
\begin{table*}[tb]
\footnotesize
\centering
\color{black}
\caption{Background of path-planning methods.} \label{tab:env}
\begin{tabular}{p{0.3cm} | p{2.5cm} | p{12.5cm}}
\textbf{No.} & \textbf{Path Planning} & \textbf{Description} \\ \toprule
1. & \textbf{Node-based} &  \\ \midrule
a. &  Centerline-based Structure (CBS) & CBS algorithm approximates the path closest to the centerline, i.e. the path that maximizes the distance from all obstacles in the environment. This method builds a tree model of the environment, where each node contains its circular/spherical approximation (i.e. position of the center and local radius from the wall). \\
b. & Depth First Search (DFS) & DFS algorithm traverses a graph by exploring as far as possible along each branch before backtracking \cite{tarjan1972depth} \\
c. &  Breadth First Search (BFS) & BFS algorithm \cite{dechter1985generalized} starts at the tree root and explores the k-nearest neighbour nodes at the present depth before moving on to the nodes at the next depth level. \\ 
d. &  Dijkstra & The Dijkstra algorithm~\cite{dijkstra1959note} is an algorithm for finding the shortest paths between nodes in a graph. It is also called Shortest Path First (SPF) algorithm. The Dijkstra algorithm explores a graph by expanding the node with minimal cost. \\
e. &  Potential field & Artificial potential field algorithms \cite{hwang1992potential} define a potential field in free space and treat the robot as a particle that reacts to forces due to these fields. The potential function is composed of an attractive and repulsive force, representing the different influences from the target and obstacles, respectively. \\
f. &  A* \& Lifelong Planning A* (LPA*) &  A-star \cite{hart1968formal} is an extension of the Dijkstra algorithm, which reduces the total number of states by introducing heuristic information that estimates the cost from the current state to the goal state. \\
g. &  Wall-following & Wall-following algorithms move parallel and keep a certain distance from the wall according to the feedback received from sensors. \\
\midrule
2. &  \textbf{Sampling-based} &  \\ \midrule
a. & Rapidly-exploring Random Tree (RRT)  & RRT \cite{lavalle1998rapidly} and its derivatives are widely used sampling-based methods. These methods randomly sample in the configuration space or workspace to generate new tree vertices and connect the collision-free vertices as tree edges. In addition, these methods can consider the kinematic constraints (i.e., curvature limitations) during MP.  \\ 
b. & Probabilistic RoadMap* (PRM*)  & A probabilistic roadmap is a network graph of possible paths in a given map based on free and occupied spaces \cite{geraerts2004comparative, karaman2011sampling}. PRM* takes random samples from the robot's configuration space, tests them for whether they are in the free space, and uses a local planner to attempt to connect these configurations to other nearby configurations. Then, the starting and goal configurations are added in, and a graph search algorithm is applied to the resulting graph to determine a path between these two configurations.  \\
\midrule
3. & \textbf{Optimisation-based} &  \\ \midrule
a. &  Mathematical Model  & \ac{MP} can be formulated as a path optimisation problem with constraints on the robot model, such as its kinematic model \cite{raja2012optimal}. The mathematical model optimizes an objective function that exists within equality and inequality constraints and is solved by linear or nonlinear programming. \\ 
b. & Evolutionary algorithms  & Evolutionary algorithms use bio-inspiration to find approximate solutions to difficult optimization problems. \ac{ACO} is one of the population-based metaheuristic algorithms \cite{dorigo2006ant}. Artificial ants incrementally build solutions biased by a pheromone model, i.e.  a set of parameters associated with graph components (either nodes or edges) whose values are modified at runtime by the ants. \ac{GA} is another bio-inspired evolutionary algorithm \cite{holland1992adaptation}, where the initial population comprises multiple chromosomes, and each chromosome is composed of several genes representing optimization variables. The population is updated by crossover and mutation of genes. Finally, the optimal solution is selected from the population after several generations. \\ \midrule
4. &  \textbf{Learning-based} &  \\ \midrule
a. & Learning from Demonstrations (LfD) & LfD is the paradigm where an agent acquires new skills by learning to imitate an expert. LfD approach is compelling when ideal behaviour cannot be easily scripted, nor defined easily as an optimisation problem, but can be demonstrated \cite{ravichandar2020recent}. \\ 
b. & Reinforcement Learning (RL) & In RL, an agent learns to maximise a specific reward signal through trial and error interaction with the environment by taking actions and observing the reward \cite{sutton2018reinforcement}. \\
\bottomrule
\end{tabular}
\end{table*}
